Delay and reliability-constrained VNF placement on mobile and volatile 5G infrastructure

The ongoing research and industrial exploitation of SDN and NFV technologies promise higher flexibility on network automation and infrastructure optimization. Choosing the location of Virtual Network Functions is a central problem in the automation and optimization of the software-defined, virtualization-based next generation of networks such as 5G and beyond. Network services provided for autonomous vehicles, factory automation, e-health and cloud robotics often require strict delay bounds and reliability constraints, which are influenced by the location of its composing Virtual Network Functions. Robots, vehicles and other end-devices provide significant capabilities such as actuators, sensors and local computation which are essential for some services. Moreover, these devices are continuously on the move and might lose network connection or run out of battery power, which further challenge service delivery in this dynamic environment. This work tackles the mobility, and battery restrictions; as well as the temporal aspects and conflicting traits of reliable, low latency service deployment over a volatile network, where mobile compute nodes act as an extension of the cloud and edge computing infrastructure. The problem is formulated as a cost-minimizing Virtual Network Function placement optimization and an efficient heuristic is proposed. The algorithms are extensively evaluated from various aspects by simulation on detailed real-world scenarios.

==> model.tex <==
\section{Model}
\label{sec:model}

%\comment{I would anticipate here that our model at the end uses inhomogeneous Mat\'ern~II~PPs as a result of considering the population and the unsuitability of Mat\'ern~I~PPs. We should make it clear here what we are aiming at.}


This section presents the model used to both generate the BSs of future MEC deployments, and to determine the locations of the MEC PoPs to which the BSs are assigned. 
In our model a BS is the first connection point in the RAN accessed by the User Equipment (UE), for example a 2G BS, a 3G NodeB, a 4G eNodeB, or a 5G gNodeB. 
In Sec.~\ref{subsec:macro-cells-generation} we extend Mat\'ern~PPs to introduce inhomogeneity and generate BSs based on the population density. 
The derived processes, namely inhomogeneous Mat\'ern~I and II~PPs, impose a minimum distance between BSs to obtain a better coverage. 
Moreover, we show that Mat\'ern~II~PPs are more suitable for BSs generation because of their relaxed thinning procedure.
Sec.~\ref{subsec:mec-pops-locations} presents the algorithm used to generate MEC PoPs that can satisfy imposed latency constraints among all the BSs that are assigned to them.

% \comment{LC: here the model should be introduced. The intuition behind the model and the approach should be described first. Otherwise it's hard to understand the following subsections.
% Basically summarize the steps, and then reference the sub-sections where the mathematical details can be found.}

\subsection{Macro cells generation}
\label{subsec:macro-cells-generation}

With the model we aim to generate more BSs in regions where the population is higher. Here we refer to a region $R$ as a subset of a complete separable metric space $\mathcal{R}$, for example a map of Spain. Hence $R$ can represent a city like Madrid and the model locates BSs in city areas where there are more people.
% \comment{LC: What is population? Human population? In the traffic model we are also considering machines. Is the traffic demand directly correlated to the population? What is a region in this case? According to the following paragraph, the region $R$ should be introduced here.}
To achieve this we consider that every region $R$ contains population circles $C_i\subset R$ defined by a center $c_i$ and a revolution function $f_i(x)$ (with $i\in[1,R_C]\cap\mathbb{N}$, and $R_C$ the number of population circles defined inside the region $R$). 
%\comment{LC: Is this $\mathcal{R}$ related to the previous $R$? They use a different font but they can be confused with each other}

The \emph{revolution function} $f_i(x)$ with $x \in C_i$ determines where it is more likely to have a person in $C_i$. 
This function leads to a surface of revolution defined at $C_i$ that can be expressed as $f_i(\lVert x - c_i \rVert_d)$,
%\comment{LC: What is the region $R$? You should introduce first what is a region $R$ before stating "Every region $R$". What is "studied location"?}
and which height expresses the amount of people at a given location $x \in R$.
Therefore, the presence of people at $x \in R $ is expressed as:
\begin{equation}
    G(x) := \sum_i f_i(\lVert x - c_i \rVert_d),\quad \forall C_i \subset R,\ \forall d\in\mathbb{N}
    \label{eq:gentrification}
\end{equation}
where $G(x)$ is referred as \emph{gentrification} in the following paragraphs.
%In this model, the \emph{revolution function} $f_i$ is the responsible of which locations will have more or less presence of population. 
%This is an advantage, since the modeling can be as complex as desired by choosing the proper $f_i$. 

\begin{figure}
    \begin{tikzpicture}
        \node[inner sep=0pt] (russell) at (0,0)
            {\includegraphics[width=\columnwidth]{revolution-function}};
        \node at (-2.2,1.1) {$f_1$};
        \node at (0.8,1.1) {$f_2$};
        \node at (-2.5,-1.1) {$C_1$};
        \node at (1.4,-1.3) {$C_2$};
        \node at (3.7, 1.1) {$G(x)$};
        \node at (-3.7,-1.4) {$R$};
    \end{tikzpicture}
    \caption{\emph{Revolution functions} of a region with two building areas.}
    \label{fig:rev}
\end{figure}

Figure~\ref{fig:rev} illustrates an example of a region $R$ with two population circles (i.e., $C_1$, $C_2$) corresponding to two distinct areas. 
Moreover, the \emph{revolution functions} $f_i$ considered in this example are Gaussian-like surfaces of revolution that can be multi lobed as the case of $f_2$, and the \emph{gentrification} function $G(x)$ is just the dashed line merging both of them.


If an \emph{inhomogeneous} PPP uses the \emph{gentrification} function $G(x)$, the process generates BSs in concordance with the population, but it is still necessary to know how many we have to generate. 
Based on~\cite{luca-5g-qos} we grid the region $R$ in cells to satisfy the imposed number of BSs per km\textsuperscript{2} in future 5G deployments, and
% \comment{LC: I wonder what's the role of the population w.r.t. the average number of antennas since.
% Moreover, I would motivating that 3GPP defines the traffic demand per square kilometer. In can be easily inferred that this would require an average number of antennas/km2.}
we take $\mathcal{R}$ as a two dimensional space where the region to be gridded $R\subset\mathcal{R}$ (for example Madrid) is expressed as a rectangle $R~=~\left[ x_{1,l}, x_{1, r} \right] \times \left[x_{2,b}, x_{2,t} \right]$ divided into cells $R_i \subset R$ of width $x_{1,s}$ and height $x_{2,s}$. The resulting grid has $w_i$ rows and $u_i$ columns that are completely determined by the cell index $i$ (which increases from left to right, and upside down as shown in Fig. \ref{fig:grid-aau-gen}):
\begin{align}
    w_i := \left\lfloor \frac{i \cdot x_{1,s}}{u_n} \right\rfloor, &\quad u_i = i\cdot x_{1,s}\mod u_n\\
                                                                   &\quad u_n = \left\lceil \frac{x_{1,s} - x_{1,l}}{x_{1,s}}\right\rceil
\end{align}
with $u_n$ being the number of columns of the gridded region~$R$.
% \comment{LC: Definitely this subsection needs to be merged with the population one. Here you give the definition of $R$, which is critical to understand all the rest. Also Fig.2 should be moved up. By moving this section up, you explain the figure from left to right, which is more natural.}
Finally, we set each cell $R_i$ as the product of two intervals $R_i~=~[x_{1,l}^i, x_{1,r}^i]\times [x_{2,b}^i, x_{2,t}^i]$ whose limits are:
\begin{align}
    x_{1,l}^i &= x_{1,l} + x_{1,s}u_i \label{eq:lim-1-l} \\
    x_{1,r}^i &= \min \left\{ x_{1,r},\ x_{1,l} + (1 + u_i)x_{1,s} \right\} \label{eq:lim-1-r} \\
    x_{2,b}^i &= \max \left\{ x_{2,b},\ x_{2,t} - (1+w_i)x_{2,s} \right\} \label{eq:lim-2-b} \\
    x_{2,t}^i &= x_{2,t} - x_{2,s}w_i \label{eq:lim-2-t}
\end{align}
\begin{figure*}[ht]
    \centering
    \input{grid.tex}
    \captionof{figure}{Gridded region on the left side, and macro cell generation inside a cell on the right side. Gray crosses without a cell tower represent BS points that did not survive after the $I_2$ \emph{thinning}. The rhs shows how the region cell $R_2$ is gridded when the repulsion radius is chosen as specified in Eq.~(\ref{eq:rep-radius}) with $N(R_2)=5$.}
    \label{fig:grid-aau-gen}
\end{figure*}
Fig.~\ref{fig:grid-aau-gen} illustrates on the left-hand side (lhs) the limiting coordinates of a region~$R$ that is gridded into cells $R_i$ according to the limits above, i.e., (\ref{eq:lim-1-l})-(\ref{eq:lim-2-t}).

In every single cell an \emph{inhomogeneous} PPP generates a specific average number of BSs using an \emph{intensity function} defined as $\lambda(x)=k\cdot G(x)$ (where $k\in\mathbb{N}$ is a constant), so BSs are located with higher probability where there are more people. 
But since we want to have the BSs as sparse as possible, it is necessary to impose a minimum distance between them. 
%Hence, inside to each cell $R_i$ a \emph{hard-core} PP is carried out.
% \comment{LC: Move the above sentence in the model Section.}
This work leverages the Mat\'ern \emph{hard-core} processes~\cite{matern} to model the BSs' generation. 
The first process under consideration for our model is the Mat\'ern I process.
\theoremstyle{definition}
\begin{definition}{Mat\'ern I point process:}
    is the point process obtained after applying a \emph{thinning} with index function:
    \begin{equation}
        I_1(x,X) := \begin{cases*}
            0 & if $N(B(x,r)) > 1$\\
            1 & if $N(B(x,r)) = 1$
        \end{cases*}
        \label{eq:matern1}
    \end{equation}
    to a \emph{stationary} PPP $X$, where $N(B(x,r))$ denotes the \emph{number of points} of the point process $X$ falling in the ball centered at $x$ with radius $r$.
    \label{def:matern1}
\end{definition}

In other words, a point $x\in X$ is removed if it has a neighbor $x' \in X$ with distance $\lVert x - x' \rVert_d < r$. 
This property suits the random generation of the BSs' locations because only one BS can be in a neighborhood.
However, these point processes are \emph{stationary} (see~\cite{stochastic-martina}), and therefore \emph{homogeneous}, before the \emph{thinning} (see Definition~\ref{def:matern1}), but this model uses \emph{inhomogeneous} PPPs to generate BSs (based on $G(x)$) at each cell $R_i\subset~R$.
%\comment{LC: It is not clear why homogeneity is not a desired property here. What's the implication? Is it related to the average number? Something else?}
Thus we modify the original definition of a \emph{Mat\'ern I} point process to use an \emph{inhomogeneous} PPP before the \emph{thinning}. 
We call these processes \emph{inhomogeneous Mat\'ern~I}~PPs.

After \emph{inhomogeneity} is introduced, we need to know an expression for the average \emph{number of points} $\mathbb{E}\left[N(C)\right]$ that can appear in a certain set $C\subset \mathcal{R}$. The reason, as shown in Proposition~\ref{prop:inh-matern1-avg}, is that this expression is in terms of the repulsion radius $r$ and the \emph{intensity function} $\lambda(x)$, and we must select these parameters accordingly to generate the desired average number of BSs in a cell~$R_i$. Since there is no expression in the literature for the average \emph{number of points} of a ``\emph{inhomogeneous Mat\'ern~I} PPs'', we have obtained it with the help of the Campbell-Mecke formula~\cite{stochastic-book}.

% \comment{LC: This explanation comes a bit out of the blue. This raise the question "Why this is not possible with homogeneous Matern processes?". We need a better transition from homogeneous to inhomogeneous processes.}

\theoremstyle{prop}
\begin{prop}
    Given an \emph{inhomogeneous} PPP $X$ with \emph{intensity function} $\lambda$, and the \emph{thinning} function $I_1$,
the resulting thinned point process, called \emph{inhomogeneous Mat\'ern~I} PP, has the following average \emph{number of points} at $C$:
    \begin{equation}
        \mathbb{E}\left[ N(C) \right] := \int_C e^{-\int_{B(x,r)} \lambda(u) du} \lambda(x)\ dx
        \label{eq:inh-matern1-avg}
    \end{equation}
    where $r$ is the \emph{thinning} radius of $I_1$.
    \label{prop:inh-matern1-avg}
\end{prop}

\begin{proof}
    First we define the auxiliary function $g$:
    \begin{align}
        g:\quad \mathcal{R} \times \Omega & \to \{0,1\}\\
(x, A) & \mapsto \mathds{1}_C(x)\ \mathds{1}\left(dist(x, X\setminus x) > r\right)
    \end{align}
    where $\Omega$ is the space of events (see~\cite{stochastic-martina}). 
    % \comment{LC: What is the space of events here?}
    We can then rewrite the average number of points at $C$ as:
    \begin{equation}
        \mathbb{E}\left[ N(C) \right] := \mathbb{E} \sum_{x \in X} g(x, X)
        \label{eq:avg-points-sum}
    \end{equation}
    Next, we use the Campbell-Mecke formula to obtain:
    \begin{gather}
        \mathbb{E}\sum_{x \in X} g(x,X) := \int_{\mathcal{R}}\mathbb{E}^x[g(x,X)]\lambda(x)\ dx =\\
        =\int_{\mathcal{R}}\int_\Omega g(x,X) \mathbb{P}^x(A)\ dA\ \lambda(x)\ dx =\\
        =\int_C \int_\Omega \mathds{1}\left(dist(x, X\setminus x) > r\right) \mathbb{P}^x(A)\ dA\ \lambda(x)\ dx =\\
        =\int_C \mathbb{P}^x\left(dist(x, X\setminus x) > r\right)\ \lambda(x) \ dx =\\
        = \int_C \mathbb{P}\left(N\left(B(x,r)\right)=0 \right)\ \lambda(x) \ dx 
    \end{gather}
    where $\mathbb{P}^x$ denotes the Palm probability. Finally, we apply the capacity functional (see~\cite{stochastic-martina}) of a PPP to obtain the stated equality.
\end{proof}
One drawback of these ``\emph{inhomogeneous Mat\'ern~I}'' processes is their very restrictive \emph{dependent thinning} procedure, which might reach the case where all the points are removed in certain neighborhoods.
To overcome such limitation, our model considers a second type of processes, known as \emph{Mat\'ern~II} point processes, that rely on \emph{marked point processes} (see~\cite{stochastic-martina}).
 \emph{Mat\'ern~II} processes assign a \emph{mark} to every point generated so as to allow the \emph{dependent thinning} processes (see~\cite{stochastic-martina}) distinguish which point is retained in a neighborhood. 

\theoremstyle{definition}
\begin{definition}{Mat\'ern II point process:}
    is the point process obtained after applying a \emph{thinning} with \emph{index function}:
    \begin{equation}
        I_2(x,m, X, M_X) := \begin{cases*}
            1 & if $m = \min_{m' \in M_X}\big\{ (x',m'):$\\
              & $\phantom{ if m = min m'} x'\in B(x,r) \big\}$\\
            0 & otherwise
        \end{cases*}
        \label{eq:matern2}
    \end{equation}
    to a \emph{stationary} \emph{marked} PPP $X$, where $M_X$ denote the marks associated to the point process $X$.
    \label{def:matern2}
\end{definition}
In other words, among all the points falling in the ball of radius $r$, only the one with the lowest mark $m$ survives.
These kind of processes present the advantage that even when the \emph{intensity function} takes high values, at least one point remains in every neighborhood. 
In our model this means that in a certain neighborhood there is no more than one BS.

If rather than using a \emph{stationary} PPP before applying the \emph{dependent thinning} $I_2$, we use an \emph{inhomogeneous} PPP (something novel in the SoA); then it is possible that the retained BS in a neighborhood is the one with higher $\lambda(x)$ by choosing the mark $(x,m)$ as $m \sim \frac{1}{\lambda(x)}$. 
% \comment{LC: based on this description, it is not clear to me whether the current state of art has ever used Mat\'ern II processes for generating the antenna locations. So far, it does not seem to me anything new (I might be wrong though).}
But still is missing how we can control that a correct number of BSs is generated at each region $R_i\subset R$ based on the repulsion radius $r$ and the \emph{intensity function} $\lambda(x)$. Thus we proceed as with the ``\emph{inhomogeneous Mat\'ern~I}''~PPs to obtain an expression for the average \emph{number of points} (something novel in the SoA).
%\comment{LC: at this point it is still unclear why we want to compute the average number of points.}

\theoremstyle{prop}
\begin{prop}
Given an \emph{inhomogeneous} marked PPP $X$ with \emph{intensity function} $\lambda$, the \emph{thinning} function $I_2$, and marks $m \sim \frac{1}{\lambda(x)}$, the resulting thinned point process, called \emph{inhomogeneous Mat\'ern~II}~PP, has the following average \emph{number of points} at $C$:
    \begin{equation}
        \mathbb{E}\left[ N(C) \right] := \int_C e^{-\int_{B(x,r)} \mathds{1}\left(\lambda(u) > \lambda(x) \right) \lambda(u) du} \lambda(x)\ dx
        \label{eq:inh-matern2-avg}
    \end{equation}
    where $r$ is the \emph{thinning} radius of $I_2$.
    \label{prop:inh-matern2-avg}
\end{prop}

\begin{proof}
    As in the proof of Proposition~\ref{prop:inh-matern1-avg}, we proceed defining the function $g$:
    \begin{align}
        g:\quad \mathcal{R} \times \Omega & \to \{0,1\}\\
        (x, A) & \mapsto \mathds{1}_C(x)\ \mathds{1}\left( \lambda(x) = \max_{x' \in X \cap B(x,r)} \left\{ \lambda(x') \right\} \right)
    \end{align}
    Then, the average number of points in a subset $C$ can be expressed as in Eq.~(\ref{eq:avg-points-sum}).
    Next, we apply the Campbell-Mecke formula as in the previous proof and we obtain the average number of points as:
    \begin{gather}
        \mathbb{E}\sum_{x\in X}g(x,X) := \int_C \mathbb{P}^x\left(\lambda(x) = \max_{x' \in X \cap B(x,r)} \right) \lambda(x)\ dx =\\
        = \int_C \mathbb{P}\left( N\left( B_{>\lambda(x)}(x,r) \right) = 0 \right) \lambda(x)\ dx =\\
        = \int_C e^{-\int_{B(x,r)} \mathds{1}\left( \lambda(u) > \lambda(x) \right) \lambda(u) du} \lambda(x)\ dx
    \end{gather}
    where $B_{>\lambda(x)}(x,r) = \left\{u: x\in B(x,r) \land \lambda(u) > \lambda(x) \right\}$ .
\end{proof}

The right-hand side (rhs) of Fig.~\ref{fig:grid-aau-gen} depicts how to obtain BSs' locations using an \emph{inhomogeneous Mat\'ern~II}~PP (whose average number of points is derived in Proposition \ref{prop:inh-matern2-avg}).
First, it generates the gray crosses using an \emph{inhomogeneous PPP} with intensity function $\lambda(x)$ (note that more points are generated on the upper right corner because of the direction of $\nabla\lambda(x)$). 
Then, a $I_2$ thinning is applied using repulsion radius $r$ with marks $m\sim\frac{1}{\lambda(x)}$, so only the gray cross with the most top-right coordinate falling within a ball of radius $r$ survive. 
This surviving cross is hence illustrated as a cell tower in Fig.{~\ref{fig:grid-aau-gen}}. 
% Don't like this explanation to tacke editorial review
%{\color{blue} The right-hand side (rhs) of Fig.~\ref{fig:grid-aau-gen} depicts how an ``\emph{inhomogeneous Mat\'ern II}'' PP generates BSs. The gray crosses are points obtained with the \emph{inhomogenous PPP} that do not survive after the $I_2$ thinning of radius $r$ is applied taking marks $m\sim\frac{1}{\lambda(x)}$ (as in Proposition \ref{prop:inh-matern2-avg}), while the drawn BSs are the ones surviving the $I_2$ thinning, and hence belonging to the \emph{inhomogeneous Mat\'ern II} PP. In this case BSs are concentrated on the top right because that is the direction of $\nabla\lambda(x)$.}

As both Propositions \ref{prop:inh-matern1-avg} and \ref{prop:inh-matern2-avg} state, the average \emph{number of points} of ``\emph{inhomogeneous} Mat\'ern~I and II''~PPs depend on the repulsion radius $r$. Then for a cell $R_i\subset~R$, we need to know which $r$ allows the generation of the required number of BSs.
% \comment{LC: the above paragraph should be rewritten when moving this section up.}
To generate $N(R_i)$ points we set the cell repulsion radius as: %\footnote{\color{red} \st{Here it is considered $x_{1,s}=x_{2,s}$ as in the experiments carried out in} Sec.~\ref{sec:results}. }

\begin{equation}
    r := \frac{2  \sqrt{x_{1,s}\cdot x_{2,s}} }{\lceil \sqrt{N(R_i)} \rceil}
    \label{eq:rep-radius}
\end{equation}
which grids $R_i$ in cells that can contain the repulsion balls $B(x,r)$ of the \emph{Mat\'ern}~PPs. 
These new cells are squares of side $2r$ and area $4r^2 > \pi r^2 = \lvert B(x,r) \rvert $, and they divide the parent cell $R_i$ in $\lceil \sqrt{N(R_i)} \rceil^2$ smaller cells that can host a whole macro cell repulsion area.



% \comment{LC: I would do the opposite, I would use this to then motivate the Matern processes, not viceversa.}

% \comment{LC: END MOVING TO HERE}

% \comment{LC: According to my understanding, the above statement is true starting from the second part of Section III.D. I would change the name of the subsection here to something more specific to the demonstration presented in Section III.D.}

% \comment{LC: I would move the Fig. 2 here. It's weird to refer to a figure that is 2 pages away.}

% \comment{LC: I propose to move this section before the presentation for Mat\'ern processes. I believe it flows better. Traffic demand -> Average number of antennas -> we define the grid -> we need a way to randomly generate the average number of antennas in each region -> Mat\'ern processes. Basically, in this section you motivate why we need the average number of antennas, while in the previous one comes out of the blue.}


% \comment{LC: enough space in the cell or region $R$? Enough space where?}
% \comment{LC: rework the above to better hook it with the Matern processes.}

% \comment{LC: be consistent. Right hand side or rhs.}

\subsection{MEC PoPs' deployment}
\label{subsec:mec-pops-locations}

We assign the traffic of every BS generated in Sec.~\ref{subsec:macro-cells-generation} to a MEC PoP that is deployed somewhere within the operators' network infrastructure, and at a specific geographic location (i.e., to minimize RTT).
The further the distance between the MEC PoP at location $m$, and a BS at location $x$, the higher the propagation delay $l(\cdot)$ of the link connecting them. The other two contributions for the packet Round Trip Time (RTT) are the radio transmission delay $t_r$ between a BS and the final user, and the packet processing delay $p(\cdot)$:
\begin{equation}
    RTT := 2 l\left(\lVert x - m \rVert_d \right) + 2 p(M) + t_r
    \label{eq:rtt}
\end{equation}
with $p(M)$ denoting the processing delay introduced by the network hops to be traversed to reach the network ring $M$. 
Hence, our model envisions the operator infrastructure as a hierarchy of network rings $\mathcal{M}$, in which traffic traverses more hops to reach network rings that are higher in the hierarchy (see Fig.~\ref{fig:infrastructure}).
That is, taking $\prec$ as a relationship expressing which network ring is higher in the network hierarchy $\mathcal{M}$, if $M_a, M_b \in \mathcal{M}$ and $M_a \prec M_b$, we can say that a MEC PoP deployed at $M_a$ is reached in less hops than one at $M_b$.
Thus, $p(M_a) < p(M_b)$, and network ring $M_a$ aggregates less traffic than $M_b$.

So if we place a MEC PoP at location $m$ and assign it to network ring $M$, after fixing the maximum RTT and radio technology, from Eq.~(\ref{eq:rtt}) we know the maximum distance to those BSs whose traffic is assigned to the new MEC PoP 
\begin{equation}
    \lVert x-m \rVert_d \le l^{-1}\left( \frac{RTT - 2p(M) - t_r}{2} \right)  = m_M
    \label{eq:max-dis}
\end{equation}
% \todo[inline]{I do not understand completely this, you are not considering routing at all, which may increase the distance and also you are not considering the capacity of the links, which may not be enough to carry the flows, even more if C-RAN is used, btw is used or not?}
Algorithm~\ref{alg:mec-pops-placement} determines the MEC PoPs' deployment in three stages:

\begin{enumerate}[leftmargin=5mm]
    \item \textbf{Initialization}: the first stage (lines \ref{alg:init-begin}-\ref{alg:init-end}) creates the set of MEC PoPs locations, the set of their network rings, the set of  BSs and one matrix of locations $x\in R$ per network ring. 
    Each entry $x$ in the matrix $matrices[M]$ represents the number of BSs that can be assigned to a MEC PoP deployed at a given location $x$ and associated to the ring $M\in \mathcal{M}$

\item \textbf{Candidates search}: this second stage (lines \ref{alg:init-mat-begin}-\ref{alg:init-mat-end}) determines how many BSs can be assigned to a MEC PoP depending on its location and associated network ring $M\in\mathcal{M}$. For every $M$ it loops through each BS and increases by one those location entries of $matrices[M]$ satisfying that if a MEC PoP is deployed there, it could satisfy the RTT and hence, the BS could be assigned to that MEC PoP. If $matrices[M_a][x_0]=4$ after this stage, it would mean that a MEC PoP associated to $M_a$ and deployed at $x_0$ would have 4 BSs assigned to itself. \label{alg-step:candidates-search}
    
    \item \textbf{MEC PoPs selection}: this third and last stage (lines \ref{alg:cover-begin}-\ref{alg:cover-end}) is the main loop of Algorithm \ref{alg:mec-pops-placement}, and each iteration decides a new MEC PoP location and network ring. \label{alg-step:mec-pops-selection}
    It comprises two phases:
        \begin{enumerate}
            \item \textbf{MEC PoP location}: this phase (lines \ref{alg:max-begin}-\ref{alg:max-end}) obtains the best location where a MEC PoP can be located. 
            It iterates through all the possible network rings in $\mathcal{M}$ searching for the location where the maximum amount of BSs can be assigned to a MEC PoP. 
            In case of having multiple locations assigning the same amount of BSs at different rings, let's call them $M_a, M_b$, then the algorithm selects the location related to the ring with the minimum propagation delay, i.e., $\min \left\{ p(M_a), p(M_b) \right\}$.
        \item \textbf{Assignment update}: the MEC PoP obtained in the previous step handles the traffic of up to maximum number of BSs \emph{ringMaxBSs()}, depending on the network ring where it is associated. Taking into account that consideration, this phase (lines \ref{alg:decrease-begin}-\ref{alg:decrease-end}) iterates through every BS assigned to the MEC PoP and updates every $matrices[M]$ to reflect the assignment by decreasing in one unit the neighborhood of each BS. That is, if the new MEC PoP has an assigned BS at location $x$, the neighboring locations of $x$ at every ring, i.e., $matrices[M][B(x,m_M)]$, must be decreased by one. Thus if another MEC PoP is latter located inside~$B(x,m_M)$, it knows that it will cover one less BS.
Finally all the assigned BSs are removed from the unassigned list.

            %\comment{LC: it is not clear what "decreases by one unit its surrounding locations at each network level matrix" means,}
            % \comment{LC: need to reword the above. Hard to understand.}
        \end{enumerate}
\end{enumerate}
Hence, Algorithm~\ref{alg:mec-pops-placement} iterates through every MEC PoP candidate location $m$, and chooses the one maximizing the number of BSs falling inside the ball $B(m,m_M)$. This process minimizes the number of MEC PoPs, and is done for every possible network ring $M$ to find the best $(m,M)$ combination.

\begin{algorithm}
 \KwData{BSs, $R$, RTT}
 \KwResult{MECPoPLocations, MECPoPRings}

 $matrices$ = array(int.matrix($R$), length = $\lvert \mathcal{M} \rvert $)\; \label{alg:init-begin}
 unassigned = Set(BSs)\;
 MECPoPLocations = Set()\;
 MECPoPRings = Set()\; \label{alg:init-end}
 \ForEach{$x$ in BSs}{ \label{alg:init-mat-begin}
     \ForEach{$M$ in $\mathcal{M}$} {
         $m_M = l^{-1}\left( \frac{RTT - 2p(M) - t_r}{2}\ \right) $ \;
         $matrices[M][B(x, m_M)]$ += 1\;
     }
 }\label{alg:init-mat-end}
 \While{not empty unassigned}{ \label{alg:cover-begin}
    covBSs = $-1$\;
    MECPoP = NULL\;
    ring = NULL\;
    \ForEach{$M \in \mathcal{M}$}{ \label{alg:max-begin}
        maxCov = $\max_{x'} \left\{ matrices[M][x'] \right\}$\;
        moreBSsCovered = $maxCov < covBSs$\;
        eQ = $\left(maxCov = covBSs \land \ p(M) < p(ring) \right)$\;
        \If{moreBSsCovered OR eQ}{
            covBSs = maxCov\;
            MECPoP = $x: matrices[M][x] = maxCov$\;
            ring = $M$\;
        }
    } \label{alg:max-end}
    MECPoPLocations.add(MECPoP)\;
    MECPoPRings.add(ring)\;
    ringMaxDis = $l^{-1}\left( \frac{RTT - 2p(ring) - t_r}{2}\ \right)$ \;
    assignBSs = BSs $\cap~B(MECPoP,\ ringMaxDis)$\; \label{alg:decrease-begin}
    \ForEach{$x \in$ assignBSs.subset(ringMaxBSs(ring))}{
        \ForEach{$M \in \mathcal{M}$}{
            $matrices[M][B(x, m_M)]$ -=1\;
        }
        unassigned.pop($x$)\;
    } \label{alg:decrease-end}
 } \label{alg:cover-end}
 \caption{MEC PoPs placement.}
 \label{alg:mec-pops-placement}
\end{algorithm}

%\subsection{MEC PoPs location [TO REMOVE]}
%\label{subsec:mec-pops-location-bad}
%{\color{red} Once the region $R$ has all the antennas' locations generated, it is possible to decide where to locate the MEC PoPs that will provide service to the traffic handled by antennas around them.

%These MEC PoPs must satisfy the delay requirements stated in \cite{3gpp} for the future 5G traffic. Among all the low-latency and high-reliability scenarios, we choose the end-to-end (E2E) latency of the tactile interaction scenario. This is the strictest E2E latency and it must be below the $0.5$ ms.

%The Round Trip Time (RTT) used in the model is}

%\begin{equation}
%    RTT \ge 2d\cdot5\frac{\mu s}{km} + 2M\cdot 50\mu s + UL + DL
%    \label{eq:rtt-bad}
%\end{equation}
%{\color{red} where $d$ stands for the distance between the MEC PoP and the BS, $5\frac{\mu s}{km}$ is the fiber optic speed, and $M$  is the number of hops introduced by the network ring \cite{luca-5g-qos} where the PoP is located. If the MEC PoP is in the access ring $M1$, then it introduces $M=1$ hop; whilst the aggregation ring $M2$ introduces $M=2$ hops. Our $RTT$ takes the packet processing time into account, which has been taken to be below $50\mu s$ \cite{eantc}. Both the first two terms in the rhs of \ref{eq:rtt-bad} stand for the propaggation delay RTT and the packet processing delay RTT, respectively. The last terms stand for the Uplink (UL) and Downlink (DL) radio delay.

%The values used for UL and DL are those of the different radio technologies that are candidates to be used in future 5G network deployments. Among the existing ones \cite{radio-delays} we have selected those that satisfy $UL + DL < RTT = 1ms$ (see Table \ref{table:radio}). The three used New Radio (NR) technologies studied use an uplink semi-persistent scheduling (SPS) framework.}

%\begin{table}
%    \centering
%    \renewcommand{\arraystretch}{1.3}
%    \begin{tabular}{ | l | l | l | l | l |}
%    \hline
%    Division & Subcarrier & Symbols & DL (ms) & UL %(ms) \\ \hline
%    FDD & 30 kHz & 2 & 0.39 & 0.39\\ \hline
%    FDD & 120 kHZ & 7 & 0.33 & 0.33\\ \hline
%    TDD & 120 kHz & 7 & 0.39 & 0.39\\
%    \hline
%    \end{tabular}
%    \caption{NR technologies satisfying the tactile experience $RTT$ shown in (\ref{eq:rtt-bad}).}
%    \label{table:radio}
%\end{table}

%{\color{red} From the UL and DL delays, together with where the MEC PoPs are located (M1 or M2); attending to (\ref{eq:rtt-bad}) one can know what is the maximum distance $d$ between the MEC PoP and the BS depending on which NR technology is used, see Table \ref{table:distances}.}

%\begin{table}
%    \centering
%    \renewcommand{\arraystretch}{1.3}
%    \begin{tabular}{ | l | l | l |}
%    \hline
%    NR & M1 distance & M2 distance  \\ \hline
%    FDD 30 kHz 2s  & 12 km & 2\phantom{0} km \\ \hline
%    FDD 120 kHZ 7s & 24 km & 14 km \\ \hline
%    TDD 120 kHz 7s &  12 km & 2\phantom{0} km\\
%    \hline
%    \end{tabular}
%    \caption{Maxmimum distance between MEC PoP and a BS depending on the used radio technology.}
%    \label{table:distances}
%\end{table}

% \begin{description}[\IEEEsetlabelwidth{Forbidden mo    ves:}\IEEEusemathlabelsep]
%     \item[]
%s \end{description}

